Fighting Uncertainty with Gradients: Offline Reinforcement Learning via Diffusion Score Matching

Gradient-based methods enable efficient search capabilities in high dimensions. However, in order to apply them effectively in offline optimization paradigms such as offline Reinforcement Learning (RL) or Imitation Learning (IL), we require a more careful consideration of how uncertainty estimation interplays with first-order methods that attempt to minimize them. We study smoothed distance to data as an uncertainty metric, and claim that it has two beneficial properties: (i) it allows gradient-based methods that attempt to minimize uncertainty to drive iterates to data as smoothing is annealed, and (ii) it facilitates analysis of model bias with Lipschitz constants. As distance to data can be expensive to compute online, we consider settings where we need amortize this computation. Instead of learning the distance however, we propose to learn its gradients directly as an oracle for first-order optimizers. We show these gradients can be efficiently learned with score-matching techniques by leveraging the equivalence between distance to data and data likelihood. Using this insight, we propose Score-Guided Planning (SGP), a planning algorithm for offline RL that utilizes score-matching to enable first-order planning in high-dimensional problems, where zeroth-order methods were unable to scale, and ensembles were unable to overcome local minima. Website: https://sites.google.com/view/score-guided-planning/home

==> abstract.tex <==
\begin{abstract}

\end{abstract}

==> body/intro.tex <==
%!TEX root = ../main.tex

\section{Introduction}

Model-based Reinforcement Learning (MBRL) is a framework where the dynamics is first learned from given data, then an optimal plan or policy is generated using the learned dynamics model \cite{atkeson,pilco}. These methods have shown promise in solving difficult tasks such as dexterous manipulation \cite{pddm}, pixel-based control \cite{carrots, e2c}, or deformable object manipulation \cite{yunzhu}. Although less asymptotically effective than model-free methods on a single task, MBRL has the advantage of being more sample efficient \cite{kaelbling,atkeson,schaal,schneider,abbeel}, and naturally generalizes to different tasks with the learned dynamics \cite{schaal, carrots}. As such, they have been a promising alternative to the sample-hungry model-free algorithms \cite{ppo, sac}. 

Yet MBRL has an important mode of failure, termed \emph{model bias} \cite{schneider, pilco, abbeel}; when the learned dynamics is put under scrutiny by powerful optimizers, the optimizers can exploit model error and give plans that do not transfer well under the real-world dynamics. Particularly, if the rollouts of the learned dynamics visit out-of-distribution (o.o.d.) regions of data, the rollouts might give a falsely optimistic solution that compromises the performance of the planner \cite{pilco, mopo}. Although this might be desirable in the online setting as it enables exploration, preventing these cases from happening is critical in the offline setting. 

To remedy these issues, previous works have proposed to use statistical uncertainty quantification \cite{calibrated,accurateuncertainty,mopo,pilco,gal2016theoretically} to identify how uncertain a result of a rollout is, and penalize the uncertainty as part of the objective function. Three popular tools used in this setting are Gaussian Processes (GP) \cite{pilco,gpmpc,glen}, bootstrapping model ensembles \cite{mopo,chua2018deep,mbtrpo}, and approximations of Bayesian inference with dropouts \cite{gal2016theoretically,gal2017concrete}. Gaussian processes show extremely promising results in low-dimensional problems \cite{pilco,glen} but rarely scale to high dimensions. On the other hand, ensembles have good scalability and have shown to have promising results in high-dimensional domains \cite{chua2018deep}. However, ensembles are prone to underestimating the true uncertainty \cite{accurateuncertainty} and can be costly to train. Methods using dropout also suffer from the similar problems of underestimating uncertainty \cite{accurateuncertainty}.

In this work, we ask the following question: \emph{is it possible to bypass the difficult problem of statistical uncertainty quantification, and directly penalize the distance to training data instead?} Intuitively, we would expect more uncertainty as we get further away from observed data. As our first contribution, we formalize this intuition by showing that distance-to-data, when scaled appropriately, is indeed an admissible estimator of uncertainty \cite{mopo} which is always guaranteed to never underestimate uncertainty. We further demonstrate that distance-to-data has a desirable property that we call \emph{data stability}: if the only objective is to minimize the proposed uncertainty metric, than doing gradient-descent on this uncertainty metric should land exactly on data. This makes data-distance a more friendly uncertainty metric in the context of gradient-based optimization; in contrast, ensembles not only fail to serve as admissible uncertainty estimators due to their tendency to underestimate, but are also prone to create spruious local minima in the uncertainty landscape.

While distance-to-data has desirable properties of being an admissible uncertainty estimator as well as data stability, its computation can be expensive to evaluate at every iteration of optimization. One may amortize this computation by directly learning this distance \cite{park2019deepsdf}. However, for large-scale datasets, this also becomes expensive as each batch has to iterate through the entire dataset to compute distance-to-data. 

Our second contribution is to effectively amortize this computation by making a connection between distance-to-data and diffusion score matching \cite{diffusion,ddpm,songscorematching}. We formalize that the softened version of distance-to-data is equivalent to the log likelihood of the \emph{perturbed data distribution}, where a small Gaussian noise is injected at each data, applying randomized smoothing \cite{duchi2012randomized,suh2022bundled} to the empirical data distribution \cite{songscorematching}. Although the exact computation of this log likelihood is expensive, its gradient (i.e. the score function) can be trained in batches using score-matching techniques \cite{songscorematching} behind recent successes in diffusion models \cite{ddpm}. Thus, we propose to learn the gradients of distance-to-data directly with score matching, and combine it with the gradient of the value function in order to penalize distance-to-data.

This connection between log likelihood of data and the softened distance-to-data also allows us to interpret penalization of distance-to-data from a divergence-minimizing perspective \cite{divergence}. We show that distance-to-data is equivalent to the the cross-entropy between the perturbed data distribution and the occupation measure of the policy (which corresponds to state-action pairs in trajectories for determinsitic open-loop plans). In contrast to existing KL-regularized approaches that penalize the divergence between the action distribution given by a stochastic policy such as behavior cloning, our approach freely allows actions to optimize reward as long as the plan stays near the data.

As our third contribution, we propose a set of algorithms for solving optimal control problems that penalize distance-to-data with diffusion score-matching, and evaluate our method on empirical examples such as the D4RL dataset \cite{d4rl}, and pixel-based planning. Importantly, we reinterpret existing approaches that utilize diffusion for planning \cite{diffusionplanning, ajay2022conditional} as a special case of our framework. We believe that this provides an elucidating interpretation behind the success of these methods, and help place it in the existing spectrum of approaches for planning in MBRL. 

In summary, our contributions are as follows:
\begin{enumerate}\itemsep -0.2em
    \item We propose distance-to-data as an alternative to statistical uncertainty estimation in MBRL.
    \item We connect distance-to-data with diffusion score matching, proposing a computationally efficient way to penalize distance-to-data in optimal planning.
    \item We show the effectiveness of our proposed algorithms on offline datasets, and reinterpret existing approaches for planning with diffusion. 
\end{enumerate}

==> body/uncertainty.tex <==
%!TEX root = ../main.tex


